A Distributed Cubic-Regularized Newton Method for Smooth Convex Optimization over Networks

We propose a distributed, cubic-regularized Newton method for large-scale convex optimization over networks. The proposed method requires only local computations and communications and is suitable for federated learning applications over arbitrary network topologies. We show a $O(k^{{-}3})$ convergence rate when the cost function is convex with Lipschitz gradient and Hessian, with $k$ being the number of iterations. We further provide network-dependent bounds for the communication required in each step of the algorithm. We provide numerical experiments that validate our theoretical results.

==> sec_experiments.tex <==
In this section, we present numerical experiments for the implementation of Algorithm~\ref{alg:main} applied to the logistic regression problem: \begin{align}\label{eq:logistic loss}
        \min_{x \in \mathbb{R}^n}\frac{1}{d}\sum\limits_{i = 1}^d \ln\Bigl(1 + \exp\bigl(-y_i\langle w_i, x \rangle\bigr)\Bigr). 
\end{align} 
We given a set of $d$ data pairs $\{y_i,w_i\}$ for $1\leq i\leq d$, where $y_i \in \{1, -1\}$ is the class label of object $i$, and $w_i \in \mathbb{R}^n$ is the set of features of object $i$. Moreover, we assume the data points are uniformly split among $m$ nodes, connected over a network, such that each node has $d^i$ data points, and $d= m\cdot d^i$.

% \begin{figure}[th!]
%     \centering
%     \includegraphics[trim=35 0 40 0, clip,width=1\linewidth]{NEW_NEW_Figure1.eps}
%     \vspace{-0.6cm}
%     \caption{\textbf{Oracle Complexity}: Optimality gap of the iterations generated by Algorithm~\ref{alg:main} for different networks topologies and different problem parameters}
%     \vspace{-0.3cm}
%     \label{fig:oracle_complex}
% \end{figure}

% \begin{wrapfigure}[20]{r}{0.5\textwidth}
% \vspace{-0.5cm}
%     \begin{minipage}{0.5\textwidth}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1\linewidth]{Figure2.eps}
%     \vspace{-0.5cm}
%     \caption{\textbf{Communication Complexity}: Consensus and optimality gap of the iterates generated by Algorithm~\ref{alg:approx_subproblem} for the solution of the auxiliary subproblems.}
%     \label{fig:comm_complex}
% \end{figure}
% \end{minipage}
% \end{wrapfigure}

\begin{figure}[th!]
    \centering
    \includegraphics[trim=35 0 40 0, clip,width=1\linewidth]{NEW_NEW_Figure1.eps}
    \vspace{-0.6cm}
    \caption{\textbf{Oracle Complexity}: Optimality gap of the iterations generated by Algorithm~\ref{alg:main} for different networks topologies and different problem parameters}
    \label{fig:oracle_complex}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.7\linewidth]{Figure2.eps}
    \caption{\textbf{Communication Complexity}: Consensus and optimality gap of the iterates generated by Algorithm~\ref{alg:approx_subproblem} for the solution of the auxiliary subproblems.}
    \label{fig:comm_complex}
\end{figure}


We compare the performance of Algorithm~\ref{alg:main} (\textbf{DecAccCubic}), centralized gradient method  (\textbf{CenGM}), distributed Newton method (\textbf{DecNewton}), distributed non-accelerated cubic method (\textbf{DecCubic}), and distributed accelerated gradient method (\textbf{DecAccGM}). See Supplementary materials for additional details. Figure~\ref{fig:oracle_complex} shows the oracle complexity of Algorithm~\ref{alg:main} in terms of the optimality gap of the generated iterations for different network topologies (Complete, Erd\"os-R\'enyi, and Cycle graphs) and various problem parameters (number of agents, number of data points and dimensions). In all scenarios we explore, the proposed approach has the best performance with respect to the oracle complexity. Figure~\ref{fig:comm_complex} shows the communication complexity of solving the auxiliary subproblems with Algorithm~\ref{alg:approx_subproblem}. The top row shows the consensus gap, which indicates that the agreement among the agents on a solution increases as the number of communication rounds increases. The bottom row shows the agreement is on a solution to the auxiliary subproblem.
